Rethinking Weight Decay for Robust Fine-Tuning of Foundation Models

Modern optimizers such as AdamW, equipped with momentum and adaptive learning rate, are designed to escape local minima and explore the vast parameter space. This exploration is beneficial for finding good loss basins when training from scratch. It is not necessarily ideal when resuming from a powerful foundation model because it can lead to large deviations from the pre-trained initialization and, consequently, worse robustness and generalization. At the same time, strong regularization on all parameters can lead to under-fitting. We hypothesize that selectively regularizing the parameter space is the key to fitting and retraining the pre-trained knowledge. This paper proposes a new weight decay technique, Selective Projection Decay (SPD), that selectively imposes a strong penalty on certain layers while allowing others to change freely. Intuitively, SPD expands and contracts the parameter search space for layers with consistent and inconsistent loss reduction, respectively. Experimentally, when equipped with SPD, Adam consistently provides better in-distribution generalization and out-of-distribution robustness performance on multiple popular vision and language benchmarks. Code available at~\url{https://github.com/GT-RIPL/Selective-Projection-Decay.git}

==> figures/pascal.tex <==
\begin{figure}[h]
     \centering
     \includegraphics[width=0.9\textwidth]{figures/pascal_pdf.pdf}
     \caption{Performance breakdown for each level of corruption on PASCAL-Context Segmentation. Models fine-tuned with SPD exhibit the best robustness against common image corruptions. }
     \label{fig:pascal}
\end{figure}

==> figures/toy.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
    \includegraphics[width=0.4\textwidth]{figures/toy_pdf.pdf}
\caption{Optimization on Himmelblau's function using Adam with SPD. Adam hyper-parameters: $\beta_1=0.9,\beta_2=0.999$. Yellow triangle: Initialization point. White stars: local minima. SPD selectively imposes regularization on the vertical direction, while horizontal traversal is free. As the regularization strength ($\lambda$) increases, Adam-SPD converges to the lower right minimum, closer to the initialization location. }
\vspace{-12mm}
\label{fig:toy}
\end{wrapfigure}

==> tables/domainet_overall.tex <==
\begin{table}
\begin{subtable}[h]{0.48\textwidth}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}[h]{c|ccccc|c}
\toprule
&\multicolumn{5}{c|}{Test Domains}\\
& Real	& Clipart &	Painting &	Sketch	&Quickdraw & Deviation\\
\midrule
Real & \color{blue}84.83 & 57.55 & 53.13 & 44.11 & 8.44& 1.53\\
\midrule
Clipart & 54.5 & \color{blue}79.88 & 40.97 & 46.87 & 13.14 & 0.83\\
\midrule
Painting & 55.62 & 46.64 & \color{blue}74.90 & 40.56 & 8.55 & 0.81  \\
\midrule
Sketch & 45.02 & 52.97 & 39.70 & \color{blue}72.26 & 15.16& 0.95 \\
\midrule
Quickdraw & 3.08 & 10.12 & 1.66 & 9.61 & \color{blue}68.68& 1.72\\
\bottomrule
\end{tabular}}
\caption{AdamW: ID Avg. 76.11, OOD Avg. 32.37}
\label{tab:adam_domainnet}
\end{subtable}
\hfill
\begin{subtable}[h]{0.48\textwidth}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}[h]{c|ccccc|c}
\toprule
&\multicolumn{5}{c|}{Test Domains}\\
& Real	& Clipart &	Painting &	Sketch	&Quickdraw & Deviation\\
\midrule
% Real & \color{blue}86.43 & 63.69 & 59.27 & 54.37 & 12.78 & 0.45 \\
Real & \color{blue}85.92 & 60.92 & 59.27 & 48.89 & 10.14 & 0.83 \\

\midrule
% Clipart & 60.16 & \color{blue}81.15 & 46.8 & 50.48 & 13 & 0.44\\
Clipart & 59.32 & \color{blue}80.75 & 45.36 & 49.89 & 12.54 & 0.55\\
\midrule
% Painting & 59.83 & 50.99 & \color{blue}77.73 & 43.95 & 3.75 & 0.42\\
Painting & 57.86 & 48.82 & \color{blue}76.95 & 42.09 & 5.75 & 0.61\\
\midrule
% Sketch & 51.85 & 56.92 & 46.16 & \color{blue}74.15 & 15.77 & 0.48\\
Sketch & 51.66 & 56.29 & 45.70 & \color{blue}73.49 & 16.43 & 0.60\\
\midrule
% Quickdraw & 15.24 & 22.2 & 10.16 & 17.37 & \color{blue}67.48 & 0.73\\
Quickdraw & 6.54 & 16.37 & 3.63 & 12.02 & \color{blue}68.91 & 0.99\\
\bottomrule
\end{tabular}}
\caption{Adam-SPD: ID Avg. \textbf{77.20}, OOD Avg. \textbf{35.47}}
\label{tab:adamspd_domainet}
\end{subtable}
\caption{Comparisons between AdamW and Adam-SPD on DomainNet. A pre-trained CLIP model is fine-tuned on each of the five domains in DomainNet and tested on all domains. Each row represents the evaluation of a model fine-tuned on a domain. The last column shows the deviation of the final model from its initialization. Adam-SPD (Tab.~\ref{tab:adamspd_domainet}) shows much better OOD performance with significantly less deviation ($\|W_t-W_0\|_2$) compared to vanilla AdamW (Tab.~\ref{tab:adam_domainnet}).}
\label{tab:domainnet}
\end{table}


==> tables/llama-13b.tex <==
\begin{table*}[h]\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{llccccccccc}
\toprule
 PEFT & Optimizer & BoolQ  &PIQA &SIQA &HellaSwag &WinoGrande &ARC-e &ARC-c &OBQA &Avg \\
 
\midrule
\multirow{2}{*}{Series}
& AdamW  &71.8&	83.0&	79.2&	88.1&	82.4&	82.5&	67.3&	81.8&	79.5 \\
&Adam-SPD\\
\midrule
\multirow{2}{*}{Parallel}
& AdamW &72.5&	84.8&	79.8&	{92.1}&	{84.7}&	84.2&	71.2& 82.4&81.5 \\
&Adam-SPD\\
\midrule
\multirow{2}{*}{LoRA}
 & AdamW&72.1&	83.5&	{80.5}&	90.5&	83.7&	82.8&	68.3& 82.4 & 80.5\\
&Adam-SPD & 72.4 & \textbf{85.6} & 80.7 & \textbf{92.4} & \textbf{86.3} & \textbf{84.5} & \textbf{71.8} & \textbf{85.2} & \textbf{82.3}\\
\bottomrule
\end{tabular}}
\caption{Accuracy comparison of LLaMA-13B with different adapters and optimizers on eight
commonsense reasoning datasets.
}
\label{tab:llama-13b}

\end{table*}

